Privacy in Foundation Models: A Conceptual Framework for System Design

AI and its relevant technologies, including machine learning, deep learning, chatbots, virtual assistants, and others, are currently undergoing a profound transformation of development and organizational processes within companies. Foundation models present both significant challenges and incredible opportunities. In this context, ensuring the quality attributes of foundation model-based systems is of paramount importance, and with a particular focus on the challenging issue of privacy due to the sensitive nature of the data and information involved. However, there is currently a lack of consensus regarding the comprehensive scope of both technical and non-technical issues that the privacy evaluation process should encompass. Additionally, there is uncertainty about which existing methods are best suited to effectively address these privacy concerns. In response to this challenge, this paper introduces a novel conceptual framework that integrates various responsible AI patterns from multiple perspectives, with the specific aim of safeguarding privacy.

==> Sec/CaseStudy.tex <==
\clearpage

\begin{figure*}[t]
\centering
\includegraphics[width=16cm]
{use-case.pdf}
\caption{The activity diagram of the hypothetical use case - a healthcare system - how each activity aligns with specific privacy goals. }
\centering
\label{use_case}
\end{figure*}

\section{A Hypothetical Use Case}\label{sec_usecase}


A hypothetical use case is presented in this section (cf. Fig.~\ref{use_case}) to show how the proposed conceptual framework might be applied. This can be used to walk through the evaluation steps in a way that brings the framework to life. Specifically, the foundation model is implemented in a healthcare management software system designed for patient engagement, record management, and diagnostic assistance.

\smallskip
\noindent\textbf{Objectives.}
This hypothetical use case proceeds through a four-step privacy evaluation framework. Our multidisciplinary team includes healthcare experts, software engineers, data scientists, privacy experts, and legal advisors. The goal is to critically assess the way the foundation model interacts with health-related and other forms of data, ensuring alignment with privacy goals specifically tailored to a healthcare context.

\smallskip
\noindent\textbf{Context.}
To present this use case in a structured manner, we follow a step-by-step walkthrough of each phase of the privacy evaluation framework. Each section elucidates how the corresponding steps align with specific privacy goals, describing the actions, decision points, and reflective activities involved. The setting for this use case is a hypothetical tech company specializing in NLP services for healthcare systems, where sensitive patient data and compliance with privacy regulations are paramount. The context provides ample room to explore multifaceted privacy challenges and demonstrates the versatility of the framework across sectors with varying degrees of complexity and sensitivity.

\smallskip
\noindent\textbf{Use cases - a healthcare system.}
In this initial phase, the team engages in a comprehensive analysis, employing privacy questionnaires and threat modeling techniques. The analysis focuses primarily on how the foundation model interacts with sensitive health records, patient demographic data, and medical histories. The goal is twofold: 1) to ensure patients are well-informed about what types of health-related data are being processed, which aligns with the goal of notice and awareness; 2) to offer opt-in or opt-out mechanisms for different levels of data processing, catering to the goal of choice and consent.

Following the insights gleaned from the initial phase, the software engineering team, in consultation with healthcare and privacy experts, suggests implementing role-based access controls. This allows patients, healthcare providers, and administrators different levels of access to sensitive health data, thus aligning with the goal of access and participation. Moreover, the system incorporates robust encryption methods to protect the health data, satisfying integrity and security.

The reflection phase introduces an additional layer of scrutiny. Ethical, legal, and technological experts interrogate the system's design decisions. For instance, while the system may employ robust encryption, the team questions if the LLM could inadvertently generate diagnostic suggestions that could be harmful or biased. This conversation aligns with the goals of enforcement and redress and even touches upon data minimization, considering whether all the collected health data is necessary for the system's operation.

Finally, all the reflections and suggestions are synthesized into a unified privacy strategy for the healthcare software system. For example, if the team identifies that too much data is being collected, stricter data retention policies focused on health data minimization might be implemented.


\smallskip
\noindent\textbf{Insights.}
The rigorous application of this privacy framework results in a healthcare management software system that is rich in nuanced, multi-dimensional privacy considerations tailored to healthcare. This elevates trust among patients, healthcare providers, and regulatory bodies. This use case serves as a robust template for similar privacy evaluations in other healthcare applications using foundation models, contributing to a healthcare industry that is more respectful of patient privacy. It also provides valuable empirical data that can inform future privacy frameworks and regulations, particularly those focusing on the unique challenges posed by the integration of AI in healthcare settings.

==> Sec/Table.tex <==
%\begin{landscape}

\begin{table*}

\centering
\tiny
\label{table_pattens}
\caption{Mapping privacy goals to RAI patterns}
\begin{tabular}{p{1.5cm}|p{2.2 cm}|p{2.2 cm}|p{6 cm}|p{4cm}}
\hline
\textbf{Conceptual Framework} & \textbf{Responsible Pattern Pool}  & \textbf{Privacy Patterns and Goals} & \textbf{Evaluation Processing}  & \textbf{Outputs} \\
\hline
\hline

 \multirow{3}{*}{\textbf{}} & \textbf{Searching}: (1) the articulation of privacy protection. & Data use limitation and purpose specification;
 
Privacy rights  & 
Searching \textbf{governance} patterns:

\begin{itemize}
    \item Industry level stakeholders and policy: engage with system solution procurers; and be aware of privacy regulation, etc;
    \item Organizational level stakeholders and standards: engage with manager and employees; and privacy standardized document patterns.
    \item Team level stakeholders and their background knowledge: engage with privacy expertise developers and end-users; and apply privacy effect analysis patterns.
\end{itemize}


 & \xmark \ Collecting excessive or unnecessary data increases the risk of data breaches exposes more sensitive information in terms of privacy, and can lead to data misuse or theft.

 \checkmark  Identify necessary data elements for system operations and which can be excluded. Reduce potential privacy risks associated with not collecting unnecessary data.

  \xmark \  Failure to identify privacy risk in the documentation and stakeholders' feedback
 \\

\cline{2-5}

\textbf{Step 1: Probing and classification of privacy requirements} (search in Fig. \ref{fig_PatternPool} pattern pool) & \textbf{Searching}: What are process patterns patterns in the pool that can be used for privacy?  & Use limitation and purpose specification;

Fairness;

Transparency & 

Search process patterns:
\begin{itemize}
    \item Search various documents in each stage, e.g., architecture documents, releases notes, and privacy unethical documents; 
    \item Search relevant privacy elements design, implementation, testing, and refactoring, and privacy basis in elicitation.
\end{itemize}
& 
\xmark \ Failure to anonymize or pseudonymize data can result in re-identification, where seemingly anonymous data can be linked back to individuals.

\checkmark \ Determine the data fields that contain sensitive information and replace or encrypt direct identifiers with pseudonyms or anonymous values.
\\
%-----------

\cline{2-5}

&  \textbf{Searching}: What are general and reusable solutions (product pattern pool) to solve a privacy issues in foundation model-based systems?  & Data minimization and storage limitation, privacy rights, data accuracy& 

Search product patterns:
\begin{itemize}
    \item  Searching product patterns that can be applied for privacy suitability assessments;
    \item  Searching for privacy user stories.
\end{itemize}

 & 

\xmark \ Absence of access controls allows unauthorized users to access sensitive data, leading to data breaches, insider threats, and unauthorized data manipulation.

\checkmark \ Define user roles and their corresponding access privileges. Categorize data based on sensitivity. Determine who should have access to different types of data.

\\
\cline{2-5}

%-------
\hline
 \multirow{3}{*}{\textbf{}} & \textbf{Suggesting}: What governance patterns are missing to establishing multi-level governance for privacy?  & Fairness;
 
 Privacy rights;
 
 & 

Suggest governance patterns:
\begin{itemize}
\item Reviewing the governance patterns that used in Step-1;
\item Suggesting and verifying the patterns that could be used for ensuring privacy.

\end{itemize}

 
 & \xmark \ Without clear comprehensive governance patterns, stakeholders struggle to navigate privacy ethical challenges, potentially leading to unethical privacy deployment and negative consequences for users.

 \checkmark  \ By suggesting specific governance patterns, the framework provides organizations with clear guidance on how to implement privacy ethical and practices. This helps them navigate complex ethical terrain and make informed decisions.
 \\

\cline{2-5}

\textbf{Step 2: Suggestive responsible patterns}: (applying patterns in Fig \ref{fig_PatternPool} pattern pool) & \textbf{Suggesting}: To suggest a set of best practices and guidelines that help ensure the responsible handling of data and the protection of user privacy throughout the development lifecycle.  & Data use limitation and purpose specification;

Fairness;

Transparency;

Data accuracy;

Pseudonymous messaging;



& Suggest the process patterns:

\begin{itemize}
    \item Privacy-focused design pattern: proposing the use of design sprints that specifically focus on privacy and ethical considerations.
    \item Data Minimization: establishing of data minimization practices
    \item User-centric privacy testing pattern: integrating of user-centric privacy testing
\end{itemize}
& 
\xmark \ The absence of process pattern can result in privacy discriminatory practices.

\checkmark \ The used patterns promote privacy by incorporating best practices and standards, ensuring that the system meets privacy and security requirements.
\\
%-----------

\cline{2-5}

&  \textbf{Suggesting}: To suggest the products patterns for systems from supply chain and system perspective.  & Ensuring transparency and fostering user trust & 

Suggest product patterns:

\begin{itemize}
    \item Data anonymity: suggesting data anonymity patterns to ensure that user identities are adequately protected by employing data anonymization and pseudonymization techniques, making it difficult to trace data back to individual users.
    \item Data encryption tool: suggesting tools to protect sensitive privacy data through encryption during transmission and storage, safeguarding it from unauthorized access and interception.
    \item Privacy impact template: suggesting to use the template for identifying and mitigating privacy risks and it also helps stakeholders assess privacy implication. 
\end{itemize}

 & 

\xmark \ The absence of product patterns can lead to inefficient resource allocation, as organizations may need to reinvent solutions for common privacy challenges in each project.

\checkmark  Product patterns offer tried-and-tested solutions to common problems, saving time and resources. Implementing patterns that prioritize privacy can enhance user trust and satisfaction, as users are more likely to engage with systems that respect their privacy.

\\

\cline{2-5}

%-------

\hline
 \multirow{3}{*}{\textbf{}} &  \textbf{Reflecting}: In assistive governance pattern usage, in this step, the framework combine probing and suggestive process to tailor the governance pattern based on the previous analysis & Enforcement and redress of privacy & 

 Reflect governance patterns:

\begin{itemize}
    \item Pattern implementation assessment: reflecting how well each governance pattern has been implemented within the system, and consider whether the intended goals are effectively translated into practice;
    \item Pattern documentation review: reflecting the documentation related to governance patterns in terms of privacy. Ensure that these documents clearly articulate the goals and processes.
    \item Stakeholder feedback: reflecting feedback from stakeholders, including privacy experts, governance board, and decision makers for circulating the privacy design.
    \item Privacy culture and awareness reflective: reflecting on the extent to which the governance patterns have contributed to building a privacy-conscious culture within the organization. Evaluate the level of privacy awareness among employees and stakeholders.
\end{itemize}

 
 &  \multirow{3}{*}{\textbf{}}


 \\

\cline{2-4}

\textbf{Step 3: Reflective pattern usage} (snowboarding more relevant patterns into the pool in Fig. \ref{fig_PatternPool}) &  \textbf{Reflecting}: Project pattern reflection involves reviewing and evaluating the patterns and practices that were applied in terms of privacy.  & Enforcement and redress of privacy & 

Reflect process patterns: 
\begin{itemize}
    \item Reflect privacy documentation: reflecting on the documentations that summarizing the outcomes of responsible pattern usage, including strength, weakness, and lessons learned. 
    \item Privacy compliance updates: reflecting that any necessary pattern usage updates are made to enhance the privacy knowledge and skills.
    \item Integration of lessons learned: reflecting to incorporate privacy lessons learned into future development iteration to build on successes. 
    \item Continuous privacy improvement: reflecting the continuous responsible patterns improvements within the development teams and emphasizing the importance of privacy driven design. 
\end{itemize}
& 
 \checkmark  Stakeholder trust: it festers trust among stakeholders, including regulatory bodies, users, data subjects and privacy ethical governance.
 
 \checkmark  Organizational learning: the reflective process contribute to organizational learning, enabling teams to draw insights from the past experience and apply them to future decision making in term of privacy.

 
 \xmark \  Non-compliance risks: failure to adapt governance patterns to changing regulations increase the risk of non-compliance with privacy laws and regulations.
\\
%-----------

\cline{2-4}

&  \textbf{Reflecting}: Product pattern usage refection includes what software artifacts and product used and their effectiveness & Enforcement and redress of privacy & Reflect product patterns: 

\begin{itemize}
    \item Reflect the success and challenges: identifying successes an challenges associated with the product patterns that applied, and determine what product patterns worked well for privacy. 
    \item Action product pattern plans: creating action plans for implementing and recommending  improvements related to product patterns. 
\end{itemize}

 & 

\\

\cline{4-4}

%-------

\hline
 \multirow{3}{*}{\textbf{}} &  \multirow{3}{*}{\textbf{}}   &  \multirow{3}{*}{\textbf{}}  & 

 & 


 \\

%\cline{4-4}

\textbf{Step 4: Combination of probing and suggestive outputs} & This step is a critical phase in the evaluation of pattern effectiveness and their real-world impact on privacy  considerations. It provides valuable insights for refining practices, ensuring compliance, and fostering a culture of responsible. & Enforcement and redress of privacy & 
Summary and suggestion based on Step-1 and Step-2:
\begin{itemize}
    \item Privacy requirement report, in this step, we document the results of privacy requirements assessment from Step 1 and 2 including a clear overview of identified data and stakeholder inputs. 
    \item Pattern usage report: documenting a report provides specific understanding what the governance, product, and process patterns have been used. In addition, it documents the how the patterns align with privacy. 
    \item Privacy road map: in this step, it also outlines steps needed to implement the recommended systems, which consist pattern recommendations to address privacy requirements, including timelines, responsible parties, and technologies. 
\end{itemize}
& 
%\xmark \ XXX

\checkmark \ Insights into the effectiveness of the suggested patterns in achieving privacy goals and ethical standards.

\checkmark  A feedback loop to integrate lessons learned from the reflective process into future projects or organizational practices.

\checkmark Recommendations for adjustments or improvements to pattern implementation based on the assessment outcomes.
\\
%-----------

%\cline{4-4}

&   &  & 



 & 

%\xmark \ XXX

%\checkmark \ XXX

\\

\cline{4-4}
%-------

%\multirow{4}{*}{\textbf{Process Pattern}} & Pattern Integration & & Integrity, Security, Enforcement, Redress & Information Transfer and Penalization & Insecure transfer and misuse of data compromise integrity and necessitate redress mechanisms. & Use secure transfer protocols, establish effective redress mechanisms & Maintained integrity, reduced infringements & \\

%\cline{2-9}

%& Testing process & &Integrity, Security, Data Minimization & Information Storage and Aggregation & Inadequate security measures and unintended sensitive data generation undermine data integrity and minimization. & Implement robust encryption, use obfuscation techniques & Enhanced security, minimized exposure & \\

%\cline{2-9}

%& Maintenance process & &Enforcement, Redress, Notice, Awareness & Information Penalization and Monitoring & Data misuse and unauthorized surveillance necessitate redress mechanisms and infringe on user awareness. & Establish effective redress mechanisms, ensure transparency & Reduced infringements, enhanced trust & \\

%\hline

%\cline{2-9}

%\hline

%-----

%& System layer & Encrypted database trainers & Integrity, Security, Data Minimization & Information Storage and Aggregation & Insufficient security measures and unintended sensitive data generation undermine data security and minimization. & Employ encrypted database training, use obfuscation techniques & Ensured confidentiality, minimized exposure & \\

%\cline{2-9}

%\multirow{2}{*}{\textbf{Product Pattern}} & Supply chain layer & Data obfuscator &Data Minimization, Access, Participation & Information Aggregation and Storage & Data aggregation and unauthorized access contradict data minimization and user control over data. & Use obfuscation techniques, implement strong access controls & Minimized exposure, improved security &\\

%\cline{2-9}

%& Operation infrastructure layer & Secure aggregator &Integrity, Security, Notice, Awareness & Information Transfer and Monitoring & Insecure transfer and unauthorized surveillance compromise data integrity and user awareness. & Use secure aggregation methods, ensure transparency & Secure aggregation, enhanced trust &\\

%\hline

%\cline{2-9}

%\hline

%-------
%& Industry level & & Notice, Awareness, Enforcement, Redress, Choice, Consent & Information Monitoring, Penalization, and Collection & Unauthorized surveillance, data misuse, and excessive data collection infringe on user rights and necessitate redress mechanisms. & Implement industry-wide standards, enforce policies on data collection & Improved industry and organization standards &\\

%\cline{2-9}

%\multirow{2}{*}{\textbf{Governance Pattern}} & Organization level & & Choice, Consent, Access, Participation, Data Minimization & Information Collection, Storage, and Aggregation & Excessive data collection, unauthorized access, and data aggregation undermine user control and data minimization. & Enforce policies on data collection, implement strong access controls, encourage minimization & Improved organization standards, enhanced team-level privacy & \\

%\cline{2-9}

%& Team level & & Data Minimization, Integrity, Security, Choice, Consent & Information Aggregation, Storage, and Collection & Data aggregation, insufficient security measures, and excessive data collection contradict minimization, compromise security, and undermine user choice. & Encourage minimization and secure practices, enforce minimization and explicit consent & Enhanced team-level privacy, reduced risk & \\
%\hline

%\cline{2-9}

\hline

\end{tabular}
\label{tab:RAIpatterns}
%\end{table}
\end{table*}




%\end{landscape}
